Three Decades of Formal Methods in Business Process Compliance: A Systematic Literature Review

Digitalization efforts often face a key challenge: business processes must not only be efficient in achieving their goals but also adhere to legal regulations. Business process compliance refers to aligning processes with these regulations. Numerous frameworks have been developed to address this, with the earliest dating back to 1981. This study focuses on rigorous frameworks using formal methods to verify or ensure compliance. We conducted a systematic literature review (SLR) on process compliance frameworks based on formal models. Our goal was to assess the current state of research on process model compliance and identify gaps and opportunities for future work. Starting with 5018 candidate studies from 1981 to the establishment of GDPR, we selected 46 primary studies. These frameworks were categorized by their phases, the languages used for processes and compliance, and their reasoning techniques. We also examined their practical applicability, the case studies they were tested on, the types of users involved, and the skills needed for compliance. Also, we assessed the maturity of each framework. Our findings reveal strong consensus around verification techniques as central to process compliance, though there is less agreement on the earlier and later phases of compliance. Model checking is the dominant technique, but the compliance and process languages have evolved. Most frameworks are still conceptual with prototype implementations, often failing to account for compliance professionals like legal experts or law changes. In conclusion, there is a need for comprehensive empirical studies to better understand the anatomy and maturity of regulatory compliance frameworks, and for robust evaluation methods to benchmark these frameworks. This review offers valuable insights for researchers and practitioners in process compliance.

==> changelog.tex <==
\section*{Changelog}


\begin{table}[h!] 
  \begin{center}
\begin{tabular}{|p{1.5cm} |p{2.5cm}|p{2.8cm}|  }
 \hline
{\bf Date} & {\bf Activity} &{\bf Participants} \\ \hline  \hline
10 November 2017 & Elaboration of first draft & 
$\begin{array}{l}
                                                  \text{Hugo A. López}
                                                  \\ \text{Søren
                                                  Debois} \\
                                                  \text{Thomas
                                                  H. Hildebrandt}
                                                \end{array}$ \\  \hline 
7 December 2017 &Expert revision and consolidation &$\begin{array}{l}
                                                       \ldots \\
                                                       \text{Barbara
                                                       Weber} \\ \text{Paolo
                                                       Tell} \end{array}$\\ \hline
20 December 2017 &Post-mortem modifications (see Appendix) & Hugo
                                                             A. López\\ \hline
 \today & Included Results from Data Analysis (see Appendix) & Hugo A.
                                                               López\\\hline
\end{tabular}
\end{center}
\end{table}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> changesAfterFinal.tex <==
\section{Changes after protocol acceptance}

The following section documents the changes suffered by the protocol
after its acceptance

\begin{itemize}
  \item Included a refined exclusion criteria:\\ - \textbf{EX5:} The
    application area of the paper does not refer to process-oriented
    technologies. \\ 
    - \textbf{EX6}: This entry is not a primary study.\\ -\textbf{ExNP}: This entry is not a full paper
    (only abstract, summary or review, etc.). \\
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> qualityAssesment.tex <==
%\section{Study quality assessment}


% \subsection{Quality checklists to be used}

% Table \ref{table:qualityChecklist} compiles the set of questions based
% on 16 issues affecting the quality of the primary study in review. 

% \begin{table}[ht!]
%   \begin{tabular}{ |p{1.2cm}||p{10cm}|p{2cm}| }
%     \hline
%     % \multicolumn{4}{|c|}{Country List} \\
%     % \hline
%     Number& Question &Measurement\\
%     \hline \hline
%     1   & What type of paper it is?    &Method/Case study\\ \hline
%     2   & How credible are the findings? (it corresponds to realistic assumptions)    &A--D Scale\\ \hline
%     3 & How well has the approach to, and formulation of analysis been
%         covered?  & A--D Scale\\ \hline
%     4 & How clear are the links between data, interpretation and
%         conclusions?  & A--D Scale\\ \hline
%     5 & How clear are the assumptions/theoretical perspectives/values
%         that have shaped the form and output of the evaluation?  & A--D
%                                                                    Scale\\    \hline
%     6 & If credible, are the findings important?  & Yes/No\\ \hline
%     7 & What is the Technology Readiness Level?  & TRL\\ \hline
%     8    &How well does the evaluation address its original aims and
%            purpose? & A--D Scale\\ \hline
%     9&   How defensible is the research design?  & A--D Scale\\ \hline
%     10& How well defined are the sample design/target selection of
%        cases/documents?  & A--D Scale \\ \hline
%     11 & Is there a prototype available?  & Yes/No\\ \hline
%     12& How well are the contexts and data sources retained and portrayed?
%                      & A--D Scale\\ \hline
%     13& How well have detail, depth, and complexity of the data been
%         covered?  & A--D Scale\\ \hline
%     14& How clear and coherent is the reporting?  & A--D Scale\\ \hline
%     15& What evidence is there of attention to ethical issues?  & A--D
%                                                                   Scale\\ \hline
%     16& How adequately has the research process been documented?  &
%                                                                     A--D
%                                                                     Scale\\
%         17& Number of Citations & Number    \\
%     \hline 
%   \end{tabular}
% \label{table:qualityChecklist}

% \end{table}
% Table \ref{table:qualityChecklist} uses the following scales:
% \begin{description}
% \item[Method/Case study]: The main contribution of the study is the
%   presentation of a method(ology) for compliance/ The main
%   contribution of the study is the presentation of a case study.
%   \item[TRL]: Technology Readiness Level (TRL) \cite{trlscale}. Each
%     of the levels describe the level of maturity of the technology in
%     question:
%     \begin{description}
%     \item[TRL 1] Basic principles observed - We will consider a
%       primary study in TRL 1 if it points out a theoretical 
%       problem and suggests possible solutions.
%     \item[TRL 2] Technology concept formulated - We will consider a
%       primary study in TRL 2 if it refers to a theory paper
%       that formulates a the solution to a theoretical problem.
%     \item[TRL 3] Experimental proof of concept - We will consider a
%       primary study in TRL  3 if it refers to a theory paper with an
%       algorithm implementing a solution proposed in TRL 2.
%     \item[TRL 4] Technology validated in lab - We will consider a
%       primary study in TRL 4 if it refers to a paper with an algorithm
%       and test runs on academic examples.
%     \item[TRL 5] Technology validated in relevant environment
%       (industrially relevant environment in the case of key enabling
%       technologies) - We will consider a
%       primary study in TRL 5 if it refers to a paper with algorithm tested on real data, but
%       not with real users. 
%     \item[TRL 6] Technology demonstrated in relevant environment
%       (industrially relevant environment in the case of key enabling
%       technologies) - We will consider a
%       primary study in TRL 6 when it refers to a paper on prototype system tested on real data
%       for real end-users, but not in real work situation.
%     \item[TRL 7] System prototype demonstration in operational
%       environment - We will consider a
%       primary study in TRL 7 when the primary study is a paper on system tested on real data for real
%       end-users in real work situation.
%     \item[TRL 8] System complete and qualified - We will consider a
%       primary study in TRL 8 when it refers to a paper on finished
%       system tested on real data for real end-users in real work
%       situation.
%     \item[TRL 9] Actual system proven in operational environment
%       (competitive manufacturing in the case of key enabling
%       technologies; or in space) - We will consider a
%       primary study in TRL 9 when it refers to a paper on finished system validated
%       in practice over time on real data for real end-users in real
%       work situation.
%     \end{description}
% Our categorisation will group the levels in pairs, to take into
% account some uncertainty. So, \textbf{TRL 1-2} will be used if the primary
% study in question is a purely theoretical paper with no sign of
% experiments. \textbf{TRL 3-4} will be used for a theory with validation on
% artificial data (e.g. made up examples). \textbf{TRL 5-6} will include primary
% studies that perform validation on real data, but not operational. \textbf{TRL
% 7-8} refers to primary studies reporting tests in operational
% environments. Finally, \textbf{TRL 9} refers to primary studies that report
% systems that have been in used for longer period and validated. For
% bookkeeping purposes we will include in the comments   quotations from
% the primary study that justify our assessment.
%   \item[A -- D Scale]: (A) Non-existent, (B) Poor, unsatisfactory evidence.  (C)
% Good, well documented evidence (D) Excellent: well-documented
% evidence, open access to data sets that justify the statement.
% \end{description}

% \subsection{ Checklist evaluation}
% All reviewers have agreed with the relevance of the questions in the
% quality checklist. 


% \subsection{ Agreement among data extractors}

% Data extraction forms will be piloted on a sample of the primary
% studies, with participation of two of the researchers involved in the
% SLR. After a first round, the instrument will be reviewed and adapted
% with the feedback reported. 

% There might be limitations on the data available for quality assessment
% in the primary sources. In case of missing data, it is responsibility
% of one of the researchers to contact the authors of the primary study
% and enquire for more information to fill the forms. 


% \subsection{ Conflict resolution}
% The primary studies will be reviewed by one of the researchers. In
% order to verify consistency in the application of the
% inclusion/exclusion criteria, the reevaluation of a random sample
% of the primary studies found after initial screening will be performed
% by a second researcher. Conflicts will be discussed and argued manually, and the
% agreement will be reported in the consolidated form. 

% \subsection{ Checklist application procedures}

% The quality data retrieved will be initially used for assisting primary
% study selection. In case the automated search retrieves more than 100
% primary studies, we will restrict the analysis to sources with
% C-D scores in questions 2, 3, 4, 5. We will call these papers
% ``high-quality papers''.  Furthermore, the quality data will be used
% to assist data analysis and synthesis, in specific, regarding
% considerations of the maturity levels of the frameworks encountered. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> schedule.tex <==
\section{Schedule}

Table \ref{table:schedule} summaries the activities required in the
construction of this SLR, as well as their expected duration.

\begin{table}[th!] 
  \begin{center}
\begin{tabular}{ |p{5cm}||p{2cm}|  }
 \hline
{\bf Activity} & {\bf Duration} \\ \hline  \hline
Construction of a review protocol & 1 month\\ \hline
Literature searching &1 month\\ \hline
Data extraction &1 month\\ \hline
Synthesis &1 month\\ \hline
Writing up &1 month\\ \hline
\end{tabular}
\caption{Schedule of the SR.}
\label{table:schedule}
\end{center}
\end{table}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

